Slender Ca II H Fibrils Mapping Magnetic Fields in the Low Solar Chromosphere

A dense forest of slender bright fibrils near a small solar active region is seen in high-quality narrowband Ca II H images from the SuFI instrument onboard the Sunrise balloon-borne solar observatory. The orientation of these slender Ca II H fibrils (SCF) overlaps with the magnetic field configuration in the low solar chromosphere derived by magnetostatic extrapolation of the photospheric field observed with Sunrise/IMaX and SDO/HMI. In addition, many observed SCFs are qualitatively aligned with small-scale loops computed from a novel inversion approach based on best-fit numerical MHD simulation. Such loops are organized in canopy-like arches over quiet areas that differ in height depending on the field strength near their roots.

==> AAS02068 <==
\begin{thebibliography}{87}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi

\bibitem[{{Ayres} {et~al.}(1986){Ayres}, {Testerman}, \& {Brault}}]{Ayres1986}
{Ayres}, T.~R., {Testerman}, L., \& {Brault}, J.~W. 1986, \apj, 304, 542

\bibitem[{{Barthol} {et~al.}(2011){Barthol}, {Gandorfer}, {Solanki},
  {Sch{\"u}ssler}, {Chares}, {Curdt}, {Deutsch}, {Feller}, {Germerott},
  {Grauf}, {Heerlein}, {Hirzberger}, {Kolleck}, {Meller}, {M{\"u}ller},
  {Riethm{\"u}ller}, {Tomasch}, {Kn{\"o}lker}, {Lites}, {Card}, {Elmore},
  {Fox}, {Lecinski}, {Nelson}, {Summers}, {Watt}, {Mart{\'{\i}}nez Pillet},
  {Bonet}, {Schmidt}, {Berkefeld}, {Title}, {Domingo}, {Gasent Blesa}, {Del
  Toro Iniesta}, {L{\'o}pez Jim{\'e}nez}, {{\'A}lvarez-Herrero},
  {Sabau-Graziati}, {Widani}, {Haberler}, {H{\"a}rtel}, {Kampf}, {Levin},
  {P{\'e}rez Grande}, {Sanz-Andr{\'e}s}, \& {Schmidt}}]{Barthol2011}
{Barthol}, P., {Gandorfer}, A., {Solanki}, S.~K., {et~al.} 2011, \solphys, 268,
  1

\bibitem[{{Berkefeld} {et~al.}(2011){Berkefeld}, {Schmidt}, {Soltau}, {Bell},
  {Doerr}, {Feger}, {Friedlein}, {Gerber}, {Heidecke}, {Kentischer},
  {von~der~L{\"u}he}, {Sigwarth}, {W{\"a}lde}, {Barthol}, {Deutsch},
  {Gandorfer}, {Germerott}, {Grauf}, {Meller}, {{\'A}lvarez-Herrero},
  {Kn{\"o}lker}, {Mart{\'{\i}}nez Pillet}, {Solanki}, \&
  {Title}}]{Berkefeld2011}
{Berkefeld}, T., {Schmidt}, W., {Soltau}, D., {et~al.} 2011, \solphys, 268, 103

\bibitem[{{Bogdan} {et~al.}(2003){Bogdan}, {Carlsson}, {Hansteen}, {McMurry},
  {Rosenthal}, {Johnson}, {Petty-Powell}, {Zita}, {Stein}, {McIntosh}, \&
  {Nordlund}}]{Bogdan2003}
{Bogdan}, T.~J., {Carlsson}, M., {Hansteen}, V.~H., {et~al.} 2003, \apj, 599,
  626

\bibitem[{{Borrero} {et~al.}(2015){Borrero}, {Jafarzadeh}, {Sch{\"u}ssler}, \&
  {Solanki}}]{Borrero2015}
{Borrero}, J.~M., {Jafarzadeh}, S., {Sch{\"u}ssler}, M., \& {Solanki}, S.~K.
  2015, \ssr, in press

\bibitem[{{Bray} {et~al.}(1991){Bray}, {Cram}, {Durrant}, \&
  {Loughhead}}]{Bray1991}
{Bray}, R.~J., {Cram}, L.~E., {Durrant}, C., \& {Loughhead}, R.~E. 1991,
  {Plasma Loops in the Solar Corona}

\bibitem[{{Bruls} \& {Solanki}(1995)}]{Bruls1995}
{Bruls}, J.~H.~M.~J. \& {Solanki}, S.~K. 1995, \aap, 293

\bibitem[{{Buente} {et~al.}(1993){Buente}, {Solanki}, \&
  {Steiner}}]{Buente1993}
{Buente}, M., {Solanki}, S.~K., \& {Steiner}, O. 1993, \aap, 268, 736

\bibitem[{Caligari {et~al.}(1995)Caligari, Moreno-Insertis, \&
  Sch{\"{u}}ssler}]{Caligari1995}
Caligari, P., Moreno-Insertis, F., \& Sch{\"{u}}ssler, M. 1995, \apj, 441, 886

\bibitem[{{Carlsson} {et~al.}(2016){Carlsson}, {Hansteen}, {Gudiksen},
  {Leenaarts}, \& {De Pontieu}}]{Carlsson2016}
{Carlsson}, M., {Hansteen}, V.~H., {Gudiksen}, B.~V., {Leenaarts}, J., \& {De
  Pontieu}, B. 2016, \aap, 585, A4

\bibitem[{{Charbonneau}(2005)}]{Charbonneau2005}
{Charbonneau}, P. 2005, Living Rev. Solar Phys., 2, 2. URL:
  http://www.livingreviews.org/lrsp

\bibitem[{{Charbonneau}(2010)}]{Charbonneau2010}
{Charbonneau}, P. 2010, Living Reviews in Solar Physics, 7, 2. URL:
  http://www.livingreviews.org/lrsp

\bibitem[{{Choudhuri}(2003)}]{Choudhuri2003}
{Choudhuri}, A.~R. 2003, in Dynamic Sun, ed. {{Dwivedi}, B.~N. and {Parker},
  F.~b.~E.~N. (Cambridge, UK: Cambridge University Press)}, 103

\bibitem[{{Danilovic} {et~al.}(2014){Danilovic}, {Hirzberger},
  {Riethm{\"u}ller}, {Solanki}, {Barthol}, {Berkefeld}, {Gandorfer}, {Gizon},
  {Kn{\"o}lker}, {Schmidt}, {Blanco Rodr{\'{\i}}guez}, \& {Del Toro
  Iniesta}}]{Danilovic2014}
{Danilovic}, S., {Hirzberger}, J., {Riethm{\"u}ller}, T.~L., {et~al.} 2014,
  \apj, 784, 20

\bibitem[{{Danilovic} {et~al.}(2010){Danilovic}, {Sch{\"u}ssler}, \&
  {Solanki}}]{Danilovic2010a}
{Danilovic}, S., {Sch{\"u}ssler}, M., \& {Solanki}, S.~K. 2010, \aap, 513, A1

\bibitem[{{de la Cruz Rodr{\'{\i}}guez} \&
  {Socas-Navarro}(2011)}]{de-laCruz2011}
{de la Cruz Rodr{\'{\i}}guez}, J. \& {Socas-Navarro}, H. 2011, \aap, 527, L8

\bibitem[{{De Pontieu} {et~al.}(2012){De Pontieu}, {Carlsson}, {Rouppe van der
  Voort}, {Rutten}, {Hansteen}, \& {Watanabe}}]{DePontieu2012}
{De Pontieu}, B., {Carlsson}, M., {Rouppe van der Voort}, L.~H.~M., {et~al.}
  2012, \apjl, 752, L12

\bibitem[{{De Pontieu} {et~al.}(2007){De Pontieu}, {McIntosh}, {Hansteen},
  {Carlsson}, {Schrijver}, {Tarbell}, {Title}, {Shine}, {Suematsu}, {Tsuneta},
  {Katsukawa}, {Ichimoto}, {Shimizu}, \& {Nagata}}]{DePontieu2007c}
{De Pontieu}, B., {McIntosh}, S., {Hansteen}, V.~H., {et~al.} 2007, \pasj, 59,
  S655

\bibitem[{{de Wijn} {et~al.}(2009){de Wijn}, {Stenflo}, {Solanki}, \&
  {Tsuneta}}]{deWijn2009}
{de Wijn}, A.~G., {Stenflo}, J.~O., {Solanki}, S.~K., \& {Tsuneta}, S. 2009,
  \ssr, 144, 275

\bibitem[{{Fontenla} {et~al.}(1993){Fontenla}, {Avrett}, \&
  {Loeser}}]{Fontenla1993}
{Fontenla}, J.~M., {Avrett}, E.~H., \& {Loeser}, R. 1993, \apj, 406, 319

\bibitem[{{Fontenla} {et~al.}(2009){Fontenla}, {Curdt}, {Haberreiter},
  {Harder}, \& {Tian}}]{Fontenla2009}
{Fontenla}, J.~M., {Curdt}, W., {Haberreiter}, M., {Harder}, J., \& {Tian}, H.
  2009, \apj, 707, 482

\bibitem[{{Gabriel}(1976)}]{Gabriel1976}
{Gabriel}, A.~H. 1976, Philosophical Transactions of the Royal Society of
  London Series A, 281, 339

\bibitem[{{Gafeira} {et~al.}(2016{\natexlab{a}}){Gafeira}, {Jafarzadeh},
  {Solanki}, {Lagg}, {van Noort}, {Barthol}, \& {Sunrise team}}]{Gafeira2016b}
{Gafeira}, R., {Jafarzadeh}, S., {Solanki}, S.~K., {et~al.} 2016{\natexlab{a}},
  \apj, submitted (this issue)

\bibitem[{{Gafeira} {et~al.}(2016{\natexlab{b}}){Gafeira}, {Solanki}, {Lagg},
  {Jafarzadeh}, {van Noort}, {Barthol}, \& {Sunrise team}}]{Gafeira2016a}
{Gafeira}, R., {Solanki}, S.~K., {Lagg}, A., {et~al.} 2016{\natexlab{b}}, \apj,
  submitted (this issue)

\bibitem[{{Gandorfer} {et~al.}(2011){Gandorfer}, {Grauf}, {Barthol},
  {Riethm{\"u}ller}, {Solanki}, {Chares}, {Deutsch}, {Ebert}, {Feller},
  {Germerott}, {Heerlein}, {Heinrichs}, {Hirche}, {Hirzberger}, {Kolleck},
  {Meller}, {M{\"u}ller}, {Sch{\"a}fer}, {Tomasch}, {Kn{\"o}lker},
  {Mart{\'{\i}}nez Pillet}, {Bonet}, {Schmidt}, {Berkefeld}, {Feger},
  {Heidecke}, {Soltau}, {Tischenberg}, {Fischer}, {Title}, {Anwand}, \&
  {Schmidt}}]{Gandorfer2011}
{Gandorfer}, A., {Grauf}, B., {Barthol}, P., {et~al.} 2011, \solphys, 268, 35

\bibitem[{{Giovanelli} \& {Jones}(1982)}]{Giovanelli1982}
{Giovanelli}, R.~G. \& {Jones}, H.~P. 1982, \solphys, 79, 267

\bibitem[{{Gudiksen} {et~al.}(2011){Gudiksen}, {Carlsson}, {Hansteen}, {Hayek},
  {Leenaarts}, \& {Mart{\'{\i}}nez-Sykora}}]{Gudiksen2011}
{Gudiksen}, B.~V., {Carlsson}, M., {Hansteen}, V.~H., {et~al.} 2011, \aap, 531,
  A154

\bibitem[{{Hayek} {et~al.}(2010){Hayek}, {Asplund}, {Carlsson}, {Trampedach},
  {Collet}, {Gudiksen}, {Hansteen}, \& {Leenaarts}}]{Hayek2010}
{Hayek}, W., {Asplund}, M., {Carlsson}, M., {et~al.} 2010, \aap, 517, A49

\bibitem[{{Henriques} \& {Kiselman}(2013)}]{Henriques2013}
{Henriques}, V.~M.~J. \& {Kiselman}, D. 2013, \aap, 557, A5

\bibitem[{{Hirzberger} {et~al.}(2011){Hirzberger}, {Feller}, {Riethm{\"u}ller},
  {Gandorfer}, \& {Solanki}}]{Hirzberger2011}
{Hirzberger}, J., {Feller}, A., {Riethm{\"u}ller}, T.~L., {Gandorfer}, A., \&
  {Solanki}, S.~K. 2011, \aap, 529, A132

\bibitem[{{Hirzberger} {et~al.}(2010){Hirzberger}, {Feller}, {Riethm{\"u}ller},
  {Sch{\"u}ssler}, {Borrero}, {Afram}, {Unruh}, {Berdyugina}, {Gandorfer},
  {Solanki}, {Barthol}, {Bonet}, {Mart{\'{\i}}nez Pillet}, {Berkefeld},
  {Kn{\"o}lker}, {Schmidt}, \& {Title}}]{Hirzberger2010}
{Hirzberger}, J., {Feller}, A., {Riethm{\"u}ller}, T.~L., {et~al.} 2010, \apjl,
  723, L154

\bibitem[{{Jafarzadeh} {et~al.}(2013){Jafarzadeh}, {Solanki}, {Feller}, {Lagg},
  {Pietarila}, {Danilovic}, {Riethm{\"u}ller}, \& {Mart{\'{\i}}nez
  Pillet}}]{Jafarzadeh2013a}
{Jafarzadeh}, S., {Solanki}, S.~K., {Feller}, A., {et~al.} 2013, \aap, 549,
  A116

\bibitem[{{Jafarzadeh} {et~al.}(2016){Jafarzadeh}, {Solanki}, {Gafeira}, {van
  Noort}, {Barthol}, {Berkefeld}, \& {Sunrise team}}]{Jafarzadeh2016b}
{Jafarzadeh}, S., {Solanki}, S.~K., {Gafeira}, R., {et~al.} 2016, \apj,
  submitted (this issue)

\bibitem[{{Jones}(1985)}]{Jones1985}
{Jones}, H.~P. 1985, in Chromospheric Diagnostics and Modelling, ed. B.~W.
  {Lites}, 175

\bibitem[{{Jones} \& {Giovanelli}(1982)}]{Jones1982}
{Jones}, H.~P. \& {Giovanelli}, R.~G. 1982, \solphys, 79, 247

\bibitem[{{Lagg} {et~al.}(2015){Lagg}, {Lites}, {Harvey}, {Gosain}, \&
  {Centeno}}]{Lagg2015}
{Lagg}, A., {Lites}, B., {Harvey}, J., {Gosain}, S., \& {Centeno}, R. 2015,
  \ssr, in press

\bibitem[{{Langangen} {et~al.}(2008){Langangen}, {De Pontieu}, {Carlsson},
  {Hansteen}, {Cauzzi}, \& {Reardon}}]{Langangen2008}
{Langangen}, {\O}., {De Pontieu}, B., {Carlsson}, M., {et~al.} 2008, \apjl,
  679, L167

\bibitem[{{Leenaarts} {et~al.}(2015){Leenaarts}, {Carlsson}, \& {Rouppe van der
  Voort}}]{Leenaarts2015}
{Leenaarts}, J., {Carlsson}, M., \& {Rouppe van der Voort}, L. 2015, \apj, 802,
  136

\bibitem[{{Lemen} {et~al.}(2012){Lemen}, {Title}, {Akin}, {Boerner}, {Chou},
  {Drake}, {Duncan}, {Edwards}, {Friedlaender}, {Heyman}, {Hurlburt}, {Katz},
  {Kushner}, {Levay}, {Lindgren}, {Mathur}, {McFeaters}, {Mitchell}, {Rehse},
  {Schrijver}, {Springer}, {Stern}, {Tarbell}, {Wuelser}, {Wolfson}, {Yanari},
  {Bookbinder}, {Cheimets}, {Caldwell}, {Deluca}, {Gates}, {Golub}, {Park},
  {Podgorski}, {Bush}, {Scherrer}, {Gummin}, {Smith}, {Auker}, {Jerram},
  {Pool}, {Soufli}, {Windt}, {Beardsley}, {Clapp}, {Lang}, \&
  {Waltham}}]{Lemen2012}
{Lemen}, J.~R., {Title}, A.~M., {Akin}, D.~J., {et~al.} 2012, \solphys, 275, 17

\bibitem[{{Linsky} \& {Avrett}(1970)}]{Linsky1970}
{Linsky}, J.~L. \& {Avrett}, E.~H. 1970, \pasp, 82, 169

\bibitem[{{Low}(1991)}]{Low1991}
{Low}, B.~C. 1991, \apj, 370, 427

\bibitem[{{Mart{\'{\i}}nez Pillet} {et~al.}(2011){Mart{\'{\i}}nez Pillet}, {Del
  Toro Iniesta}, {{\'A}lvarez-Herrero}, {Domingo}, {Bonet}, {Gonz{\'a}lez
  Fern{\'a}ndez}, {L{\'o}pez Jim{\'e}nez}, {Pastor}, {Gasent Blesa}, {Mellado},
  {Piqueras}, {Aparicio}, {Balaguer}, {Ballesteros}, {Belenguer}, {Bellot
  Rubio}, {Berkefeld}, {Collados}, {Deutsch}, {Feller}, {Girela}, {Grauf},
  {Heredero}, {Herranz}, {Jer{\'o}nimo}, {Laguna}, {Meller}, {Men{\'e}ndez},
  {Morales}, {Orozco Su{\'a}rez}, {Ramos}, {Reina}, {Ramos},
  {Rodr{\'{\i}}guez}, {S{\'a}nchez}, {Uribe-Patarroyo}, {Barthol}, {Gandorfer},
  {Kn{\"o}lker}, {Schmidt}, {Solanki}, \& {Vargas
  Dom{\'{\i}}nguez}}]{Martinez-Pillet2011}
{Mart{\'{\i}}nez Pillet}, V., {Del Toro Iniesta}, J.~C., {{\'A}lvarez-Herrero},
  A., {et~al.} 2011, \solphys, 268, 57

\bibitem[{Moreno-Insertis(1986)}]{Moreno-Insertis1986}
Moreno-Insertis, F. 1986, \aap, 166, 291

\bibitem[{{Nordlund}(1982)}]{Nordlund1982}
{Nordlund}, A. 1982, \aap, 107, 1

\bibitem[{{Ossendrijver}(2003)}]{Ossendrijver2003}
{Ossendrijver}, M. 2003, \aapr, 11, 287

\bibitem[{{Pereira} {et~al.}(2012){Pereira}, {De Pontieu}, \&
  {Carlsson}}]{Pereira2012}
{Pereira}, T.~M.~D., {De Pontieu}, B., \& {Carlsson}, M. 2012, \apj, 759, 18

\bibitem[{{Pesnell} {et~al.}(2012){Pesnell}, {Thompson}, \&
  {Chamberlin}}]{Pesnell2012}
{Pesnell}, W.~D., {Thompson}, B.~J., \& {Chamberlin}, P.~C. 2012, \solphys,
  275, 3

\bibitem[{{Pietarila} {et~al.}(2009){Pietarila}, {Hirzberger}, {Zakharov}, \&
  {Solanki}}]{Pietarila2009}
{Pietarila}, A., {Hirzberger}, J., {Zakharov}, V., \& {Solanki}, S.~K. 2009,
  \aap, 502, 647

\bibitem[{{Reardon} \& {Cauzzi}(2012)}]{Reardon2012}
{Reardon}, K.~P. \& {Cauzzi}, G. 2012, in American Astronomical Society Meeting
  Abstracts, Vol. 220, American Astronomical Society Meeting Abstracts 220,
  201.11

\bibitem[{{Rempel}(2014)}]{Rempel2014}
{Rempel}, M. 2014, \apj, 789, 132

\bibitem[{{Riethm{\"u}ller} {et~al.}(2016){Riethm{\"u}ller}, {Solanki},
  {Barthol}, {Gandorfer}, {Gizon}, \& {Sunrise team}}]{Riethmuller2016}
{Riethm{\"u}ller}, T.~L., {Solanki}, S.~K., {Barthol}, P., {et~al.} 2016, \apj,
  submitted (this issue)

\bibitem[{{Riethm{\"u}ller} {et~al.}(2013){Riethm{\"u}ller}, {Solanki},
  {Hirzberger}, {Danilovic}, {Barthol}, {Berkefeld}, {Gandorfer}, {Gizon},
  {Kn{\"o}lker}, {Schmidt}, \& {Del Toro Iniesta}}]{Riethmuller2013c}
{Riethm{\"u}ller}, T.~L., {Solanki}, S.~K., {Hirzberger}, J., {et~al.} 2013,
  \apjl, 776, L13

\bibitem[{{Roberts}(1990)}]{Roberts1990}
{Roberts}, B. 1990, Washington DC American Geophysical Union Geophysical
  Monograph Series, 58, 113

\bibitem[{{Rosenthal} {et~al.}(2002){Rosenthal}, {Bogdan}, {Carlsson}, {Dorch},
  {Hansteen}, {McIntosh}, {McMurry}, {Nordlund}, \& {Stein}}]{Rosenthal2002}
{Rosenthal}, C.~S., {Bogdan}, T.~J., {Carlsson}, M., {et~al.} 2002, \apj, 564,
  508

\bibitem[{{Rouppe van der Voort} \& {de la Cruz
  Rodr{\'{\i}}guez}(2013)}]{Rouppe2013}
{Rouppe van der Voort}, L. \& {de la Cruz Rodr{\'{\i}}guez}, J. 2013, \apj,
  776, 56

\bibitem[{{Rouppe van der Voort} {et~al.}(2009){Rouppe van der Voort},
  {Leenaarts}, {de Pontieu}, {Carlsson}, \& {Vissers}}]{Rouppe2009}
{Rouppe van der Voort}, L., {Leenaarts}, J., {de Pontieu}, B., {Carlsson}, M.,
  \& {Vissers}, G. 2009, \apj, 705, 272

\bibitem[{{Rutten}(2006)}]{Rutten2006}
{Rutten}, R.~J. 2006, in Astronomical Society of the Pacific Conference Series,
  Vol. 354, Solar MHD Theory and Observations: A High Spatial Resolution
  Perspective, ed. J.~{Leibacher}, R.~F. {Stein}, \& H.~{Uitenbroek}, 276

\bibitem[{{Rutten} {et~al.}(2004){Rutten}, {de Wijn}, \&
  {S{\"u}tterlin}}]{Rutten2004}
{Rutten}, R.~J., {de Wijn}, A.~G., \& {S{\"u}tterlin}, P. 2004, \aap, 416, 333

\bibitem[{{Rutten} {et~al.}(2015){Rutten}, {Rouppe van der Voort}, \&
  {Vissers}}]{Rutten2015}
{Rutten}, R.~J., {Rouppe van der Voort}, L.~H.~M., \& {Vissers}, G.~J.~M. 2015,
  \apj, 808, 133

\bibitem[{{Schad} {et~al.}(2013){Schad}, {Penn}, \& {Lin}}]{Schad2013}
{Schad}, T.~A., {Penn}, M.~J., \& {Lin}, H. 2013, \apj, 768, 111

\bibitem[{{Schou} {et~al.}(2012){Schou}, {Scherrer}, {Bush}, {Wachter},
  {Couvidat}, {Rabello-Soares}, {Bogart}, {Hoeksema}, {Liu}, {Duvall}, {Akin},
  {Allard}, {Miles}, {Rairden}, {Shine}, {Tarbell}, {Title}, {Wolfson},
  {Elmore}, {Norton}, \& {Tomczyk}}]{Schou2012}
{Schou}, J., {Scherrer}, P.~H., {Bush}, R.~I., {et~al.} 2012, \solphys, 275,
  229

\bibitem[{{Schrijver} \& {Title}(2003)}]{Schrijver2003}
{Schrijver}, C.~J. \& {Title}, A.~M. 2003, \apjl, 597, L165

\bibitem[{Sch{\"{u}}ssler {et~al.}(1994)Sch{\"{u}}ssler, Caligari, Ferriz-Mas,
  \& Moreno-Insertis}]{Schussler1994}
Sch{\"{u}}ssler, M., Caligari, P., Ferriz-Mas, A., \& Moreno-Insertis, F. 1994,
  \aap, 281, L69

\bibitem[{{Sekse} {et~al.}(2012){Sekse}, {Rouppe van der Voort}, \& {De
  Pontieu}}]{Sekse2012}
{Sekse}, D.~H., {Rouppe van der Voort}, L., \& {De Pontieu}, B. 2012, \apj,
  752, 108

\bibitem[{{Sekse} {et~al.}(2013){Sekse}, {Rouppe van der Voort}, {De Pontieu},
  \& {Scullion}}]{Sekse2013b}
{Sekse}, D.~H., {Rouppe van der Voort}, L., {De Pontieu}, B., \& {Scullion}, E.
  2013, \apj, 769, 44

\bibitem[{{Skumanich} {et~al.}(1975){Skumanich}, {Smythe}, \&
  {Frazier}}]{Skumanich1975}
{Skumanich}, A., {Smythe}, C., \& {Frazier}, E.~N. 1975, \apj, 200, 747

\bibitem[{{Solanki}(1993)}]{Solanki1993}
{Solanki}, S.~K. 1993, \ssr, 63, 1

\bibitem[{{Solanki}(2001)}]{Solanki2001}
{Solanki}, S.~K. 2001, in ASP Conf. Ser. (San Francisco: ASP), Vol. 248,
  Magnetic Fields Across the Hertzsprung-Russell Diagram, ed. {{Mathys}, G. and
  {Solanki}, S.~K. and {Wickramasinghe}, D.~T.}, 45

\bibitem[{{Solanki} {et~al.}(2010){Solanki}, {Barthol}, {Danilovic}, {Feller},
  {Gandorfer}, {Hirzberger}, {Riethm{\"u}ller}, {Sch{\"u}ssler}, {Bonet},
  {Mart{\'{\i}}nez Pillet}, {del Toro Iniesta}, {Domingo}, {Palacios},
  {Kn{\"o}lker}, {Bello Gonz{\'a}lez}, {Berkefeld}, {Franz}, {Schmidt}, \&
  {Title}}]{Solanki2010}
{Solanki}, S.~K., {Barthol}, P., {Danilovic}, S., {et~al.} 2010, \apjl, 723,
  L127

\bibitem[{{Solanki} {et~al.}(2006){Solanki}, {Inhester}, \&
  {Sch{\"u}ssler}}]{Solanki2006}
{Solanki}, S.~K., {Inhester}, B., \& {Sch{\"u}ssler}, M. 2006, Rep. Prog. in
  Phys., 69, 563

\bibitem[{{Solanki} {et~al.}(2016){Solanki}, {Riethm{\"u}ller}, {Barthol},
  {Danilovic}, {Deutsch}, {Doerr}, {Feller}, {Gandorfer}, \& {Sunrise
  team}}]{Solanki2016}
{Solanki}, S.~K., {Riethm{\"u}ller}, T.~L., {Barthol}, P., {et~al.} 2016, \apj,
  submitted (this issue)

\bibitem[{{Solanki} \& {Steiner}(1990)}]{Solanki1990}
{Solanki}, S.~K. \& {Steiner}, O. 1990, \aap, 234, 519

\bibitem[{{Solanki} {et~al.}(1991){Solanki}, {Steiner}, \&
  {Uitenbroeck}}]{Solanki1991}
{Solanki}, S.~K., {Steiner}, O., \& {Uitenbroeck}, H. 1991, \aap, 250, 220

\bibitem[{{Spruit}(1981)}]{Spruit1981b}
{Spruit}, H.~C. 1981, NASA Special Pub., 450, 385

\bibitem[{{Stenflo}(1989)}]{Stenflo1989}
{Stenflo}, J.~O. 1989, \aapr, 1, 3

\bibitem[{{Stenflo}(2012)}]{Stenflo2012}
{Stenflo}, J.~O. 2012, \aap, 547, A93

\bibitem[{{Uitenbroek}(2001)}]{Uitenbroek2001}
{Uitenbroek}, H. 2001, \apj, 557, 389

\bibitem[{{van Noort} {et~al.}(2005){van Noort}, {Rouppe van der Voort}, \&
  {L{\"o}fdahl}}]{vanNoort2005}
{van Noort}, M., {Rouppe van der Voort}, L., \& {L{\"o}fdahl}, M.~G. 2005,
  \solphys, 228, 191

\bibitem[{{V{\"o}gler} \& {Sch{\"u}ssler}(2007)}]{Voegler2007}
{V{\"o}gler}, A. \& {Sch{\"u}ssler}, M. 2007, \aap, 465, L43

\bibitem[{{V{\"o}gler} {et~al.}(2005){V{\"o}gler}, {Shelyag}, {Sch{\"u}ssler},
  {Cattaneo}, {Emonet}, \& {Linde}}]{Voegler2005}
{V{\"o}gler}, A., {Shelyag}, S., {Sch{\"u}ssler}, M., {et~al.} 2005, \aap, 429,
  335

\bibitem[{{Wedemeyer-B{\"o}hm} {et~al.}(2009){Wedemeyer-B{\"o}hm}, {Lagg}, \&
  {Nordlund}}]{Wedemeyer-Bohm2009}
{Wedemeyer-B{\"o}hm}, S., {Lagg}, A., \& {Nordlund}, {\AA}. 2009, \ssr, 144,
  317

\bibitem[{{Wiegelmann} {et~al.}(2016){Wiegelmann}, {Neukirch}, {Nickeler},
  {Solanki}, {Barthol}, {Gandorfer}, \& {Sunrise team}}]{Wiegelmann2016}
{Wiegelmann}, T., {Neukirch}, T., {Nickeler}, D.~H., {et~al.} 2016, \apj,
  submitted (this issue)

\bibitem[{{Wiegelmann} {et~al.}(2015){Wiegelmann}, {Neukirch}, {Nickeler},
  {Solanki}, {Mart{\'{\i}}nez Pillet}, \& {Borrero}}]{Wiegelmann2015}
{Wiegelmann}, T., {Neukirch}, T., {Nickeler}, D.~H., {et~al.} 2015, \apj, 815,
  10

\bibitem[{{Wiegelmann} {et~al.}(2010){Wiegelmann}, {Solanki}, {Borrero},
  {Mart{\'{\i}}nez Pillet}, {del Toro Iniesta}, {Domingo}, {Bonet}, {Barthol},
  {Gandorfer}, {Kn{\"o}lker}, {Schmidt}, \& {Title}}]{Wiegelmann2010}
{Wiegelmann}, T., {Solanki}, S.~K., {Borrero}, J.~M., {et~al.} 2010, \apjl,
  723, L185

\bibitem[{{Wiegelmann} {et~al.}(2013){Wiegelmann}, {Solanki}, {Borrero},
  {Peter}, {Barthol}, {Gandorfer}, {Mart{\'{\i}}nez Pillet}, {Schmidt}, \&
  {Kn{\"o}lker}}]{Wiegelmann2013}
{Wiegelmann}, T., {Solanki}, S.~K., {Borrero}, J.~M., {et~al.} 2013, \solphys,
  283, 253

\bibitem[{{Wiegelmann} {et~al.}(2008){Wiegelmann}, {Thalmann}, {Schrijver}, {De
  Rosa}, \& {Metcalf}}]{Wiegelmann2008}
{Wiegelmann}, T., {Thalmann}, J.~K., {Schrijver}, C.~J., {De Rosa}, M.~L., \&
  {Metcalf}, T.~R. 2008, \solphys, 247, 249

\bibitem[{{Zhang} \& {Zhang}(2000)}]{Zhang2000}
{Zhang}, M. \& {Zhang}, H. 2000, \solphys, 194, 29

\end{thebibliography}

